Unifying Inference for Bayesian and Petri Nets

Recent work by the authors equips Petri occurrence nets (PN) with probability distributions which fully replace nondeterminism. To avoid the so-called confusion problem, the construction imposes additional causal dependencies which restrict choices within certain subnets called structural branching cells (s-cells). Bayesian nets (BN) are usually structured as partial orders where nodes define conditional probability distributions. In the paper, we unify the two structures in terms of Symmetric Monoidal Categories (SMC), so that we can apply to PN ordinary analysis techniques developed for BN. Interestingly, it turns out that PN which cannot be SMC-decomposed are exactly s-cells. This result confirms the importance for Petri nets of both SMC and s-cells.

==> cat.tex <==
% !TEX root =  main.tex

\section{Categorical Conditional Probabilities for Petri Nets}

Similar categorical analysis methods are useful and natural also for probabilistic Petri nets.

Objects are integers.

A branching cells from a m- to an n-marking is an arrow (a rectangular matrix) from $2^m$ to $2^n$. Rows and columns are assignments (yes or no) of initial and final places. The entry gives the conditional probability.

Sequential and parallel compositions build an arrow corresponding to the entire Petri net. It gives the probability that  the corresponding marking is inhabited or not.

Notice that we DO NOT get the probability distribution on maximal configurations. To obtain it we would need a termination place for each maximal configuration.

